Software Compartmentalization Trade-Offs with Hardware Capabilities

Compartmentalization is a form of defensive software design in which an application is broken down into isolated but communicating components. Retrofitting compartmentalization into existing applications is often thought to be expensive from the engineering effort and performance overhead points of view. Still, recent years have seen proposals of compartmentalization methods with promises of low engineering efforts and reduced performance impact. ARM Morello combines a modern ARM processor with an implementation of Capability Hardware Enhanced RISC Instructions (CHERI) aiming to provide efficient and secure compartmentalization. Past works exploring CHERI-based compartmentalization were restricted to emulated/FPGA prototypes. In this paper, we explore possible compartmentalization schemes with CHERI on the Morello chip. We propose two approaches representing different trade-offs in terms of engineering effort, security, scalability, and performance impact. We describe and implement these approaches on a prototype OS running bare metal on the Morello chip, compartmentalize two popular applications, and investigate the performance overheads. Furthermore, we show that compartmentalization can be achieved with an engineering cost that can be quite low if one is willing to trade off on scalability and security, and that performance overheads are similar to other intra-address space isolation mechanisms.

==> Makefile <==
TARGET=paper
SRC=paper.tex sections/00-abstract.tex sections/02-background.tex \
	sections/04-implementation.tex sections/06-related_work.tex \
	sections/01-introduction.tex sections/03-design.tex \
	sections/05-evaluation.tex sections/07-conclusion.tex

dvi: all

all:
	pdflatex --draftmode -shell-escape $(TARGET)
	bibtex $(TARGET)
	pdflatex -shell-escape $(TARGET)
	pdflatex -shell-escape $(TARGET)

show:
	latexmk -pvc $(TARGET)


spellcheck:
	$(foreach f,$(SRC), aspell -l EN_US -t -c $(f) -p ./.aspell.txt;)

clean:
	latexmk -c

superclean: clean
	latexmk -C


==> sections/challenges.tex <==
\section{Challenges}
The following section examines the challenges faced by compartmentalization within a single address space on the Morello platform in hybrid mode. Sharing data between isolated compartments is a major challenge. We outline potential solutions in the context of performance and engineering cost considerations.

\subsection{Sharing Data}
Pointers to data which is now private to a compartment, cannot be dereferenced successfully by design. However, this raises issues for most compartment models: \textit{how to selectively share data?} Pointers are used in many applications and libraries as a way of avoiding the cost of copying data when arguments are passed, this is done for performance reasons.

\subsection{Replacing pointers with capabilities}
Morello capabilities grant controlled, bounded access to data which is not within bounds of a compartment \textit{DDC}. This removes the need to share data through other mechanisms such as shared data regions and eliminates the potential for oversharing data. Pointers can be changed to capabilities by using compiler annotations (Listing \ref{lst:cap_annotation}). This approach could be extended to an unlimited number of compartments, since capabilities are used in the same way as pointers.


\begin{tcolorbox}[colback=lightgrey,boxrule=0pt,arc=0pt,left=6pt]
{
\begin{lstlisting}[caption={Example of compiler annotation needed to change pointer to capability.},captionpos=b, label={lst:cap_annotation}]
struct stat *statbuf; // pointer
struct stat *__capability statbuf; // capability
 \end{lstlisting}

}
\end{tcolorbox}
\subsubsection{Engineering Cost}
This solution is only amenable to small scenarios such as at a function level because the cost of mixing pointer and capabilities can become burdensome. Consider the following scenario: \texttt{Compartment 1: SQLite, Compartment 2: vfscore + ramfs, Default Compartment: everything else}. Now consider the following path of execution: \texttt{findInodeInfo}\textit{(SQLite, Comp1)} -> \texttt{fstat}, \textit{(vfscore, Comp2)} -> \texttt{sys\_fstat}, \textit{(vfscore, Comp2)} -> \texttt{vfs\_fstat}, \textit{(vfscore, Comp2)} -> \texttt{vn\_stat}, \textit{(vfscore, Comp2)} -> \texttt{memset}, \textit{(libc, Default)}. In this scenario, a struct is allocated on the stack in compartment 1, a pointer is then passed through compartment 2, and used in the default compartment (\texttt{memset}). This would require the developer to modify a libc function to now accept a capability argument. To do so would also require rewriting all other calls to \texttt{memset}.

\subsubsection{Performance Cost}
Avoiding the need to copy data to a region of shared memory, or sharing through other mechanisms means that the performance cost is low.

\subsubsection{Shared data region with overlap}
This approach is the similar to the one taken by MPK~\cite{FlexOS}. Here, a region of memory is reserved to contain shared data. For static variables, an annotation is used to relocate it at link time. Dynamically allocated data is allocated into shared data by a shared data allocator. Since capability bounds must cover contiguous memory, the shared data region is located between two compartments in memory. Their \textit{DDC} bounds are extended to cover this region, so granting both access to shared data, illustrated in Figure \ref{fig:2comps}. This approach only works for two compartments.

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{diagrams/2complayout.drawio.png}
\caption{Compartment bounds when a shared memory region is used. The compartment bounds overlap to encompass shared data.}
\label{fig:2comps}
\end{figure}

\subsubsection{Engineering Cost}
The effort needed to identify shared data is in many cases lower than propagating capabilities through a system, with only annotations needed to indicate to the FlexOS toolchain which data should be regarded as such. An experienced developer can do this with fairly low effort.

\subsubsection{Performance Cost}
The only performance cost associated with this approach, is where stack variables must now be transformed into allocated shared data heap variables, with the associated cost of an allocation.

\subsection{Exception based shared data access}
Access to shared data is normally limited by compartment bounds, making the approach only applicable to two compartments. However, exception based shared data access reserves a register to hold a capability granting access to the shared data region, we selected \texttt{c18} to do this. Upon attempted access to shared data via pointer, a capability bounds fault is triggered, at which point the compartment \textit{DDC} and shared data capability in \texttt{c18} are swapped, granting access to shared data, this is illustrated in Figure \ref{fig:exceptions}. When compartment data is accessed, the same happens. As a result, this approach can extend to more compartments.

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{diagrams/exception_switch.drawio.png}
\caption{Exception based shared data access approach. \textit{DDC} before and after a capability bounds fault when attempting to access shared data.}
\label{fig:exceptions}
\end{figure}

\subsubsection{Engineering Cost}
Engineering cost is similar to that of the previous approach, except that there may now be more compartments to identify shared data.

\subsubsection{Performance Cost}
Relying on exceptions to switch \textit{DDC} is a costly approach~\cite{thekkath1994hardware}. For this reason, we did not evaluate this approach further in this paper.



==> sections/design_mod.tex <==
\section{Design: FlexOS on CHERI Hybrid Mode}


We propose two design approaches suitable for hybrid compartments on Morello, guided by four main considerations: the engineering effort to retrofit compartmentalization in existing software, compartmentalization's performance overhead, the security of the given approach and how it scales to many compartments.

\paragraph{Low Engineering Effort}
Engineering efforts are a significant barrier to the adoption of compartmentalization, as they increase costs and development complexity.
Achieving low engineering efforts can be broken down into two requirements.
First, implemented systems must be POSIX compliant to have maximum compatibility with widely used legacy code bases which are not easily modified or ported to new systems and architectures.
Second, most existing software is written with assumptions and trust models which often do not consider compartmentalization~\cite{conffuzz}, and can make compartmentalizing such code bases challenging.
Solutions must, therefore, make this transition as easy as possible.

\paragraph{Low Performance Overhead}
Performance in software systems often comes at the cost of security~\cite{underbridge}, this is because additional checks and verification add overhead to a minimal, performance optimized system.
Conversely, high performance costs are a significant barrier to the adoption of compartmentalization~\cite{ERIM, norton2016hardware}.
Thus, performance overheads should be minimal in relation to the security gains achieved.
The recent DARPA CPM call~\cite{darpa} specified this to be <5\% for application level compartmentalization with function granularity compartments.
Higher overhead is allowed for proportionally higher security gains.

\paragraph{Security}
Security is a spectrum of guarantees over an uncompartmentalized system. The precise security requirements must be judged against the other requirements to strike an acceptable balance. As a minimum, solutions must enforce strong isolation between compartments and provide access to only a subset of data which has been selectively shared.

\paragraph{Scalability}
How scalable a proposed solution is, impacts how easily it can be deployed in a system with many compartments as well as the specific design considerations which are made by the implementing developer. For example, when implementing a mechanism in which only easily extends to a few compartments, the developer must make certain design considerations such as prioritizing which components need to be compartmentalized.


\subsection{Design Overview}
\label{def:switcher}
Addressing the detailed considerations, we have selected FlexOS~\cite{FlexOS} to implement a prototype system for evaluation.
FlexOS' design enables the easy compartmentalization of legacy code, having been designed with isolation and security as primary concerns.
Furthermore, it is based upon a POSIX compatible LibOS, Unikraft~\cite{unikraft}, which will greatly improve the adoptablility of the system, with popular and widely used applications such as SQLite, available and compatible.
This also enables easier comparison to other isolation mechanisms.
Since LibOSes such as FlexOS and Unikraft are highly specialised, they also maximise performance by minimising the inclusion of unnecessary code and libraries.
This also serves to minimise the attack surface presented.

Compartments are defined statically at build time in the linker script, using a configuration file provided to the build tool~\cite{FlexOS}.
Global compartment capabilities are initialised at boot time based on these defined boundaries.
Once the developer has defined their compartment scheme, gates are inserted in place of function calls, where these calls now cross compartment boundaries.
Gates are the beginning of the switching process, and are used to invoke the switcher, when then performs the domain switching, including switching the stack and global compartment capabilities.
Finally, a trampoline function is called, which branches to the desired function.
The switcher and global compartment capabilities cannot be accessed by compartments directly, instead they must use a sealed capability.
The switching mechanism is kept as lightweight as possible to minimize overhead while preserving strong security.
All data is treated as private compartment data, unless it is specifically annotated and thus shared.
Similarly to FlexOS~\cite{FlexOS}, we define the trusted computing base as the early boot code, memory manager, scheduler, interrupt handler, along with the Morello backend.


\subsection{Approaches To Sharing Data}

Pointers to data which is now private to a compartment, cannot be dereferenced successfully by design.
However, this raises issues for most compartment models: \textit{how to selectively share data?} Pointers are used in many applications and libraries as a way of avoiding the cost of copying data when arguments are passed, this is done for performance reasons. As a result, designing an efficient and performant data sharing mechanism which scales well, preserves good security properties and does not present a major engineering hurdle for implementing developers, is crucial.

\subsubsection{Replacing pointers with capabilities}
Morello capabilities grant controlled, bounded access to data which is not within bounds of a compartment \textit{DDC}.
This removes the need to share data through other mechanisms such as shared data regions and eliminates the potential for oversharing data.
Pointers can be changed to capabilities by using compiler annotations (Listing \ref{lst:cap_annotation}).
This approach could be extended to an unlimited number of compartments, since capabilities are used in the same way as pointers.


%\begin{tcolorbox}[colback=lightgrey,boxrule=0pt,arc=0pt,left=6pt]
%{
\begin{lstlisting}[backgroundcolor = \color{lightgray},
                   language = C,caption={Example of compiler annotation needed to change pointer to capability.},captionpos=b, label={lst:cap_annotation}]
struct stat *statbuf; // pointer
struct stat *__capability statbuf; // capability
 \end{lstlisting}
 
 \paragraph{Trust Model}
Here, the trust model is a sandbox model, where the isolated function represents the distrusted compartment and is isolated from the rest of the system. Pointer arguments entering the compartment are replaced with capabilities which restrict the bounds of the external data accesses. The rest of the system is assumed to be trusted in this model and can access any memory within the sandbox compartment.

%}
%\end{tcolorbox}
\textbf{Engineering Cost} 
This solution is only amenable to small scenarios such as at the function level because the cost of mixing pointer and capabilities can become burdensome.
Consider the following scenario: \texttt{Compartment 1: SQLite, Compartment 2: vfscore + ramfs, Default Compartment: everything else}.
Now consider the following path of execution: \texttt{findInodeInfo}\textit{(SQLite, Comp1)} -> \texttt{fstat}, \textit{(vfscore, Comp2)} -> \texttt{sys\_fstat}, \textit{(vfscore, Comp2)} -> \texttt{vfs\_fstat}, \textit{(vfscore, Comp2)} -> \texttt{vn\_stat}, \textit{(vfscore, Comp2)} -> \texttt{memset}, \textit{(libc, Default)}.
In this scenario, a struct is allocated on the stack in compartment 1, a pointer is then passed through compartment 2, and used in the default compartment (\texttt{memset}).
This would require the developer to modify a libc function to now accept a capability argument.
To do so would also require rewriting all other calls to \texttt{memset}.

\textbf{Performance Cost} 
Avoiding the need to copy data to a region of shared memory, or sharing through other mechanisms means that the performance cost is low.

\textbf{Security}
The sandbox is isolated by the \textit{PCC} and \textit{DDC}, constraining all legacy data access. In addition, any shared data is tightly bounded by argument capabilities resulting in strong isolation.

\textbf{Scalability} 
This approach scales easily to an unlimited number of compartments with the effort for each additional annotated component being constant, not growing in complexity.

\subsubsection{Shared data region with overlap}
This approach is the similar to the one taken by MPK~\cite{FlexOS}.
Here, a region of memory is reserved to contain shared data.
For static variables, an annotation is used to relocate it at link time.
Dynamically allocated data is allocated into shared data by a shared data allocator.
Since capability bounds must cover contiguous memory, the shared data region is located between two compartments in memory.
Their \textit{DDC} bounds are extended to cover this region, so granting both access to shared data, illustrated in Figure \ref{fig:2comps}.

\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{diagrams/2complayout.drawio.pdf}
\caption{Compartment bounds with shared memory regions. The compartment bounds overlap to encompass shared data.}
\label{fig:2comps}
\end{figure}

\paragraph{Trust Model}
Mutual distrust is enforced between compartments, with none able to access the others' private data.


\textbf{Engineering Cost} 
The effort needed to identify shared data is in many cases lower than propagating capabilities through a system, with only annotations needed to indicate to the FlexOS toolchain which data should be regarded as such.
An experienced developer can do this with fairly low effort.

\textbf{Performance Cost} 
The only performance cost associated with this approach, is where stack variables must now be transformed into allocated shared data heap variables, with the associated cost of an allocation. The data shadow stack technique implemented on FlexOS~\cite{FlexOS} could not be implemented due to the contiguity requirement of DDC bounds.

\textbf{Security}
In the same way as the sandbox model, isolation of legacy memory access is enforced by the compartment \textit{PCC} and \textit{DDC}. Data sharing is however at a coarser granularity with the entire shared memory accessible to all compartments creating the potential for oversharing.

\textbf{Scalability} 
This approach only scales to two compartments without additional compiler support, as a result the requirement for contiguous capability bounds. Extending this approach to more compartments which need to access the same shared data would result in the inclusion of distrusting compartments in the \textit{DDC} bounds.





==> sections/models.tex <==
\section{Compartmentalization Models}
We now describe the compartmentalization models which have been evaluated. These are broader library isolation, and finer grained function sandboxing.

\subsection{Library Isolation}
The library isolation model supports two compartments, and data sharing is done via a shared data region of memory. Data is allocated into this region and compartment \textit{DDCs} overlap in this region to give both access to shared data. This model has been implemented with SQLite, with \texttt{vfscore} and \texttt{ramfs} isolated in the second compartment.

\subsubsection{Threat Model}
In this model, there is mutual distrust between compartments, hence for this model, the only overlap in \textit{DDCs} occurs at the shared data region.

\subsection{Function Sandboxing}
Sandboxed functions are modified to enable passing in and use of capabilities. This requires more effort but results in a sandboxed function which is only able to access external data via tightly bounded capabilities. To avoid the need to rewrite each function call to a sandboxed function, a wrapper is called to create bounded capabilities and then call the sandboxed function passing in capabilities. A sandboxed function returns pointers.

Under the hood, this translates into a function being in a compartment in much the same way as libraries in other models. We evaluate this model using sandboxed Libsodium functions.

\subsubsection{Threat Model}
A sandboxed function is distrusted. It resides within the capability bounds of the main compartment. This means that the main compartment is able to access data within the sandboxed function, but the sandboxed function is not able to dereference pointers which point outside the sandbox. This is useful for a function which is at risk of being compromised. Isolation is tightly enforced by \textit{DDC} bounds.

==> sections/requirements.tex <==
\section{Requirements}
In the following section we examine the key design considerations, engineering and performance costs, which are needed for successful and adoptable compartmentalization and how we can approach the design of the system. Evaluation of our implementation will also take into consideration the costs associated with both.

\subsection{Key Design Considerations}
\subsubsection{Low Engineering Effort}
Engineering cost can be a significant barrier to adoption of compartmentalization, since a high engineering effort will mean that the time to deploy is longer, and the cost is higher. A low engineering effort is crucial to drive adoption. Low engineering effort can be broken down into smaller requirements. Firstly, an implemented system must be POSIX compliant to have maximum compatibility with widely used legacy code bases which are not easily modified or ported to new systems and architectures. Secondly, most existing software is written with assumptions and trust models which often do not consider compartmentalization~\cite{conffuzz}, and can make compartmentalizing such code bases challenging. Solutions must, therefore, make this transition as easy as possible.

\subsubsection{Acceptable Performance Overhead}
Performance in software systems often comes at the cost of security~\cite{underbridge}, this is because additional checks and verification add overhead to a minimal, performance optimized system. When considering performance, it is important to examine an acceptable range of performance overheads, in relation to the security gained through compartmentalization. Any solution implemented must minimize performance overhead.

\subsection{Approach}
Addressing both engineering and performance considerations, we have selected FlexOS~\cite{FlexOS} to implement a prototype system for evaluation. FlexOS was designed to enable the easy compartmentalization of legacy code, having been designed with isolation and security as primary concerns. Furthermore, it is based upon a POSIX compatible LibOS, Unikraft~\cite{unikraft}, which will greatly improve the adoptablility of the system, with popular and widely used applications such as SQLite, available and compatible. This also enables easier comparison to other isolation mechanisms. Since libOSes such as FlexOS and Unikraft are highly specialized, they also maximize performance by minimizing the inclusion of unnecessary code and libraries. This also serves to minimize the attack surface presented.

